OpenCL Performance Prediction using Architecture-Independent Features

OpenCL is an attractive model for heterogeneous high-performance computing systems, with wide support from hardware vendors and significant performance portability. To support efficient scheduling on HPC systems it is necessary to perform accurate performance predictions for OpenCL workloads on varied compute devices, which is challenging due to diverse computation, communication and memory access characteristics which result in varying performance between devices. The Architecture Independent Workload Characterization (AIWC) tool can be used to characterize OpenCL kernels according to a set of architecture-independent features. This work presents a methodology where AIWC features are used to form a model capable of predicting accelerator execution times. We used this methodology to predict execution times for a set of 37 computational kernels running on 15 different devices representing a broad range of CPU, GPU and MIC architectures. The predictions are highly accurate, differing from the measured experimental run-times by an average of only 1.2%, and correspond to actual execution time mispredictions of 9 {\mu}s to 1 sec according to problem size. A previously unencountered code can be instrumented once and the AIWC metrics embedded in the kernel, to allow performance prediction across the full range of modelled devices. The results suggest that this methodology supports correct selection of the most appropriate device for a previously unencountered code, which is highly relevant to the HPC scheduling setting.

==> ieee-author-preamble.latex <==
\author{\IEEEauthorblockN{Beau Johnston}
\IEEEauthorblockA{\textit{Research School of Computer Science} \\
\textit{Australian National University}\\
Canberra, Australia \\
beau.johnston@anu.edu.au}
\and
\IEEEauthorblockN{Greg Falzon}
\IEEEauthorblockA{\textit{School of Science and Technology} \\
\textit{University of New England}\\
Armidale, Australia \\
gfalzon2@une.edu.au}
\and
\IEEEauthorblockN{Josh Milthorpe}
\IEEEauthorblockA{\textit{Research School of Computer Science} \\
\textit{Australian National University}\\
Canberra, Australia \\
josh.milthorpe@anu.edu.au}
}


==> templates/acm-longtable-fix-preamble.latex <==
\makeatletter
\let\oldlt\longtable
\let\endoldlt\endlongtable
\def\longtable{\@ifnextchar[\longtable@i \longtable@ii}
\def\longtable@i[#1]{\begin{figure}[t]
\onecolumn
\begin{minipage}{0.5\textwidth}
\oldlt[#1]
}
\def\longtable@ii{\begin{figure}[t]
\onecolumn
\begin{minipage}{0.5\textwidth}
\oldlt
}
\def\endlongtable{\endoldlt
\end{minipage}
\twocolumn
\end{figure}}
\newcommand{\removelatexerror}{\let\@latex@error\@gobble}
\xpatchcmd{\@todo}{\setkeys{todonotes}{#1}}{\setkeys{todonotes}{inline,#1}}{}{}
\newtoggle{ACM-BUILD}
\toggletrue{ACM-BUILD}
\makeatother



==> templates/ieee-longtable-fix-preamble.latex <==
\makeatletter
\let\oldlt\longtable
\let\endoldlt\endlongtable
\def\longtable{\@ifnextchar[\longtable@i \longtable@ii}
\def\longtable@i[#1]{\begin{figure}[t]
\onecolumn
\begin{minipage}{0.5\textwidth}
\oldlt[#1]
}
\def\longtable@ii{\begin{figure}[t]
\onecolumn
\begin{minipage}{0.5\textwidth}
\oldlt
}
\def\endlongtable{\endoldlt
\end{minipage}
\twocolumn
\end{figure}}
\newcommand{\removelatexerror}{\let\@latex@error\@gobble}
\xpatchcmd{\@todo}{\setkeys{todonotes}{#1}}{\setkeys{todonotes}{inline,#1}}{}{}
\newtoggle{IEEE-BUILD}
\toggletrue{IEEE-BUILD}
\newtoggle{ACM-BUILD}
\togglefalse{ACM-BUILD}
\newtoggle{LNCS-BUILD}
\togglefalse{LNCS-BUILD}
\makeatother
\lstset{frame=tb, tabsize=4, showstringspaces=false, numbers=none, commentstyle=\color{blue}, keywordstyle=\color{green}, stringstyle=\color{red}, basicstyle=\ttfamily\footnotesize, xleftmargin=3.4pt, xrightmargin=3.4pt}
\captionsetup[table]{name=table}

